CompHEP - a package for evaluation of Feynman diagrams and integration over multi-particle phase space. User's manual for version 33

CompHEP is a package for automatic calculations of elementary particle decay and collision properties in the lowest order of perturbation theory (the tree approximation). The main idea prescribed into the CompHEP is to make available passing on from the Lagrangian to the final distributions effectively with a high level of automation.

==> guide/output/form.tex <==


The structure of the \FORM~ \cite{FORM}  output is similar to those of
\REDUCE~ and 
\MATHEMATICA~ described above.  In the case of \FORM~ output a  
default summation  is not implemented 
and the user  must write  {\it UserSum()} anyway. 
An incomplete  sample of such procedure is written to 
 {\it  usr{\sc N}.frm}. In its turn this file is read  from  
{\it sum{\sc N}.frm}. Here N is the subprocess ordering number.
The denominator  factors (\ref{denominator}) are   presented in the form of functions 

{\tt den(-p1-p2,0,2)}
\\
where the first argument is a momentum of virtual particle, the second one is
the particle mass identifier, and the third one is the power of propagator. 

 
Unfortunately the \CompHEP~ group has not got too much  experience with 
the \FORM~ package 
and now this output cannot be commented well enough.
It was created as a result of D.Bardin's request and was used
by him and his co-authors for semi-analytic calculations.  Please, look at
these  files and try to understand how the \FORM~ output  can be used by you.

